UBC-DLNLP at SemEval-2023 Task 12: Impact of Transfer Learning on African Sentiment Analysis

We describe our contribution to the SemEVAl 2023 AfriSenti-SemEval shared task, where we tackle the task of sentiment analysis in 14 different African languages. We develop both monolingual and multilingual models under a full supervised setting (subtasks A and B). We also develop models for the zero-shot setting (subtask C). Our approach involves experimenting with transfer learning using six language models, including further pertaining of some of these models as well as a final finetuning stage. Our best performing models achieve an F1-score of 70.36 on development data and an F1-score of 66.13 on test data. Unsurprisingly, our results demonstrate the effectiveness of transfer learning and fine-tuning techniques for sentiment analysis across multiple languages. Our approach can be applied to other sentiment analysis tasks in different languages and domains.

==> langsinmodels.tex <==
\begin{table*}[!h]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{ll}
\hline
\textbf{Language Model} &\textbf{African languages represented} \\   \hline
%MT5 & Afrikaans, Chichewa, Hausa, Igbo, Shona, Somali, Sotho, Swahili, Xhosa, Yoruba, Zulu.  \\ 
%MBART & Afrikaans,Swahili, Yoruba. \\
MBERT & Afrikaans, Malagasy, Swahili, Yoruba \\
XLM-R & Afrikaans, Amharic, Hausa, Oromo, Somali, Swahili, Xhosa. \\ \hline
AfriBERTA & Afaan Oromoo, Amharic, Gahuza, Hausa, Igbo, Nigerian Pidgin, Somali, Swahili, Tigrinya and Yoruba \\
%AfriVeTa & Afaan Oromoo, Amharic, Gahuza, Hausa, Igbo, Nigerian Pidgin, Somali, Swahili, Tigrinya, and Yoruba. \\
Afro-XLMR &  Afrikaans, Amharic, Hausa, Igbo, Malagasy, Chichewa, Oromo, Nigerian Pidgin, Kinyarwanda, Kirundi, \\
& Shona, Somali, Sesotho, Swahili, isiXhosa, Yoruba, and isiZulu \\
& Luo, Moore, Chewa, Nigerian Pidgin, Shona, Swahili, Setswana, Akan Twi, Wolof, Xhosa, Yoruba, IsiZulu \\
\hline
\textbf{\ourmodel} & Includes 517 African languages.\\\hline
\end{tabular}
}
\caption{Encoder-only models with African languages represented \cite{serengeti_2022}.}
\label{tab:resources}

\end{table*}

==> models.tex <==
\begin{table*}[h!]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{lccccccc}
\hline
\multicolumn{1}{c}{}                                 & \multicolumn{2}{c}{\textbf{Vocabulary}}                                    & \multicolumn{1}{c}{} & \multicolumn{1}{c}{}    & \multicolumn{3}{c}{\textbf{Training Data}}                                                                          \\\cline{2-3}   \cline{6-8} 
\multicolumn{1}{l}{\multirow{}{}{\textbf{Model}}} & \multicolumn{1}{c}{\textbf{Tok}} & \multicolumn{1}{c}{\textbf{Vocab Size}} & \multicolumn{1}{c}{\multirow{}{}{\textbf{\#Params}}}      & \multicolumn{1}{c}{\multirow{}{}{\textbf{\#Lang.} (afr/all)}} & \multicolumn{1}{c}{\textbf{Tokens} (afr/all)} & \multicolumn{1}{c}{\textbf{Size} (afr/all)} & \multicolumn{1}{c}{\textbf{Source}} \\
\hline
xlmr                                            & SP                               & 250k                                    & 270M                                      & 8 / 100                                       & UNK/164B                                & UNK/2.4 GB                            & CC-100                                            \\
mbert                                           & WP                               & 110K                                    & 110M                                      & 4 / 100                                       & UNK/12.8B                               & UNK/100GB                             & Books, Wiki.                                      \\ \midrule
Afro-XLMR                                       & SP                               & 70.6K                                   &270M                                      & 17 / 20                                       & ---                                 & 21.6 GB                           & mC4, CC, BBC, VOA                                 \\
AfriBERTa                                       & WP                               & 70k                                     & 111M                                      & 11 / 11               & 108.8M                              & 0.94 GB                           & BBC, CC                   \\\midrule
Serengeti                                            & SP                               & 250K                                    & 278M                                         & 517/527                                     & 7.1B/8.6B                                &40/42GB		                               & RT, News, GD, HD, EC   \\                            
\hline
\end{tabular}}%}
\caption{Models with African languages that we finetune. SP: SentencePiece, WP: WordPiece. Data sources include - CC: CommonCrawl, EC: Existing corpora, GD: Government documents, HD: Health documents, RT: Religious text, UNK: Unknown \cite{serengeti_2022}.}
\label{tab:encoder-only}
\end{table*}
